Intrinsic Harmonization for Illumination-Aware Compositing

Despite significant advancements in network-based image harmonization techniques, there still exists a domain disparity between typical training pairs and real-world composites encountered during inference. Most existing methods are trained to reverse global edits made on segmented image regions, which fail to accurately capture the lighting inconsistencies between the foreground and background found in composited images. In this work, we introduce a self-supervised illumination harmonization approach formulated in the intrinsic image domain. First, we estimate a simple global lighting model from mid-level vision representations to generate a rough shading for the foreground region. A network then refines this inferred shading to generate a harmonious re-shading that aligns with the background scene. In order to match the color appearance of the foreground and background, we utilize ideas from prior harmonization approaches to perform parameterized image edits in the albedo domain. To validate the effectiveness of our approach, we present results from challenging real-world composites and conduct a user study to objectively measure the enhanced realism achieved compared to state-of-the-art harmonization methods.

==> figures/albedo_harm_dataset.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{images/albedo_harm_dataset.jpg}
    
    \resizebox{0.5\textwidth}{!}{
    }
    \caption{Example images edits used to train the Albedo Harmonization model. We randomly edit the original albedo to create a naive composite albedo that does not match its environment. We train the network to recover the original albedo therefore learning to match the foreground with the environment.}
    \label{fig:supp:harmdataset}
\end{figure}

==> figures/userstudypage.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/userstudypage.png}
    \caption{The instruction page of our user study. Image credit: Unsplash users Jean-Philippe Delberghe and Miguel Constantin Montes}
    \label{fig:userstudypage}
\end{figure}

==> tables/albedonet_params.tex <==
\begin{table}[t]
\caption{Edit operation definition and the parameter ranges used to generate naive composite training images for the albedo matching network.}
\resizebox{\linewidth}{!}
{
\begin{tabular}{l|lc}
             Operation          & Formulation &  Parameter range \\
             \hline             
             Exposure           &   $ I' =  p_{exp} \cdot I $                           & $[0.5, 2]$   \\
             Saturation         &   $ I'=RGB(h,p_{sat}\times s ,v) \quad$ h,s,v=HSV(I)         & $[0, 2]$    \\
             Color curve        &   As defined by ~\citet{hu2018exposure}                               & $[0.5, 2]$ \\
             White balance    &   $ I' =  p_{wb} \cdot I $ (channel-wise)             & $[0.3, 0.7]$    \\
\end{tabular}
}
\label{tab:albedonet:params}
\end{table}

==> tex/0_abstract.tex <==

Despite significant advancements in network-based image harmonization techniques, there still exists a domain disparity between typical training pairs and real-world composites encountered during inference. Most existing methods are trained to reverse global edits made on segmented image regions, which fail to accurately capture the lighting inconsistencies between the foreground and background found in composited images. In this work, we introduce a self-supervised illumination harmonization approach formulated in the intrinsic image domain. First, we estimate a simple global lighting model from mid-level vision representations to generate a rough shading for the foreground region. A network then refines this inferred shading to generate a harmonious re-shading that aligns with the background scene. In order to match the color appearance of the foreground and background, we utilize ideas from prior harmonization approaches to perform parameterized image edits in the albedo domain. To validate the effectiveness of our approach, we present results from challenging real-world composites and conduct a user study to objectively measure the enhanced realism achieved compared to state-of-the-art harmonization methods. 
